Enumeration Algorithms for Conjunctive Queries with Projection

We investigate the enumeration of query results for an important subset of CQs with projections, namely star and path queries. The task is to design data structures and algorithms that allow for efficient enumeration with delay guarantees after a preprocessing phase. Our main contribution is a series of results based on the idea of interleaving precomputed output with further join processing to maintain delay guarantees, which maybe of independent interest. In particular, for star queries, we design combinatorial algorithms that provide instance-specific delay guarantees in linear preprocessing time. These algorithms improve upon the currently best known results. Further, we show how existing results can be improved upon by using fast matrix multiplication. We also present new results involving tradeoff between preprocessing time and delay guarantees for enumeration of path queries that contain projections. Boolean matrix multiplication is an important query that can be expressed as a CQ with projection where the join attribute is projected away. Our results can therefore also be interpreted as sparse, output-sensitive matrix multiplication with delay guarantees.

==> spaceresult1.tex <==

\section{Space-Delay Tradeoffs}

In this section, we will present our main results for tradeoffs between space required by the data structure constructed during a preprocessing phase and the delay guarantee achieved during the enumeration phase for a subset of acyclic queries. Before we present the main results, we review some previously known algorithms. We will mainly be interested in path queries (and more generally any acyclic query with at most two projection variables). We denote the path query by
%
\begin{equation*} 
\pathq(x_1, \dots, x_{k+1}) = R_1(x_1, x_2),R_2(x_2, x_3), \dots,R_k(x_k, x_{k+1})
\end{equation*}
%
The simplest way to evaluate $\pathq(D)$ is to compute the full join query result and then de-duplicate. This approach takes $O(|D|^{\rho^*})$ time where $\rho^* = \lceil k/2 \rceil$. The next proposition improves upon this baseline result.

\begin{proposition} \label{prop:space:one}
	Consider query $\pathq$ and any input database instance $D$. Then, there exists an algorithm that can preprocess $D$ in time and space,
	\begin{align*}
	T_p = {O}(|D|^2) \quad \quad S_p = {O}(|D|^2)
	\end{align*}
	such that we can enumerate $\ell$ tuples of $Q(D)$ with
	\begin{align*}
	\text{delay } \delta = O(1) \quad \quad \text{space } S_e = O(1)
	\end{align*}
\end{proposition}
\begin{proof}
	We construct the following query decomposition. The root bag consists of $x_1, x_2, x_k, x_{k+1}$. The child of root bag consists of variables $x_2, x_3, x_{k-1}, x_k$. We continue in a similar manner. Figure tbd shows the decomposition. It is easy to see that all variables are connected and each relation belongs to at least one bag. Since the fractional hypertree width $\fhw = 2$, one can materialize all the bags in $O(|D|^2)$ time and space. We then perform a semi-join pass to eliminate any dangling tuples. At the end of semi-join phase, the root bag will contain only those tuples such that there is a reachable path from $x_1, x_2$ to $x_k, x_{k+1}$. At this point, it is safe to project away variables $x_2, x_k$ and remove any duplicate tuples. The enumeration phase then simply enumerate all tuples in the root bag without any duplication. This concludes the proof.
\end{proof}	

\autoref{prop:basic:one} requires a very expensive preprocessing phase that takes $O(|D|^2)$ time. On the hand,~\autoref{prop:basic:two} already tells us we can achieved linear delay with linear time preprocessing. For heirarchical queries,~\autoref{thm:basic:three} gives the following tradeoff $S_p = O(|D|^{1+(\mw-1) \epsilon})$ and delay $\delta = O(|D|^{1-\epsilon})$. However, what happens when we have unlimited preprocessing time but only limited space $S_p$? We present result of two flavors in this section: $(i)$ we show that for acyclic query with at most two projection variables (including path query $\pathq$), there exists a linear tradeoff between space and delay (\autoref{subsec:first:space}). We then further improve the space requirement of the data structure via a more clever degree partitioning argument (\autoref{subsec:second:space}); $(ii)$ we present a data structure for hierarchical queries that is better compared to~\cite{kara19} with respect to space usage (\autoref{subsec:third:space}).

\subsection{Warmup} \label{subsec:first:space}

In this section, we state the first result for space-delay tradeoffs followed by its proof.

\begin{theorem} \label{thm:space:one}
	Consider an arbitrary acyclic query $Q$ with at most two projection variables and a database $D$. Then, there exists a data structure that requires space $S = O(|D|^2/\delta)$ which can be used to enumerate the results of $Q(D)$ with delay $\delta$.
\end{theorem}

Remarkably,~\autoref{thm:space:one} does not exhibit any dependence on the size of the query. This is in direct contrast to previous work~\cite{deep2018compressed} where the goal was to check whether any fixing of valuations for variables leads to a join result or not. Without loss of generality, we assume that the projection variables are in different atoms (otherwise the problem is trivial).

\begin{figure}
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,222.921875); %set diagram left start at 0, and has height of 222.921875

%Shape: Ellipse [id:dp3099374396386705] 
\draw [color={rgb, 255:red, 11; green, 48; blue, 238 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]   (124,52) .. controls (124,40.95) and (139.67,32) .. (159,32) .. controls (178.33,32) and (194,40.95) .. (194,52) .. controls (194,63.05) and (178.33,72) .. (159,72) .. controls (139.67,72) and (124,63.05) .. (124,52) -- cycle ;
%Shape: Ellipse [id:dp9074469639131073] 
\draw [color={rgb, 255:red, 11; green, 48; blue, 238 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]   (150,112) .. controls (150,100.95) and (165.67,92) .. (185,92) .. controls (204.33,92) and (220,100.95) .. (220,112) .. controls (220,123.05) and (204.33,132) .. (185,132) .. controls (165.67,132) and (150,123.05) .. (150,112) -- cycle ;
%Shape: Ellipse [id:dp358822605747638] 
\draw [color={rgb, 255:red, 11; green, 48; blue, 238 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]   (183,194) .. controls (183,182.95) and (198.67,174) .. (218,174) .. controls (237.33,174) and (253,182.95) .. (253,194) .. controls (253,205.05) and (237.33,214) .. (218,214) .. controls (198.67,214) and (183,205.05) .. (183,194) -- cycle ;
%Straight Lines [id:da5929312959509521] 
\draw    (159,72) -- (177.5,91.92) ;


%Straight Lines [id:da41837202792321126] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (120.5,71.92) -- (88.5,99.92) ;


%Straight Lines [id:da14928348395329905] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (107.5,176.92) -- (75.5,206.92) ;


%Straight Lines [id:da08257282175415015] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (326.5,116.92) -- (290.5,94.92) ;


%Straight Lines [id:da26077196950121473] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (267.5,140.92) -- (231.5,118.92) ;


%Shape: Ellipse [id:dp008497036537579827] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] (216,79) .. controls (216,67.95) and (231.67,59) .. (251,59) .. controls (270.33,59) and (286,67.95) .. (286,79) .. controls (286,90.05) and (270.33,99) .. (251,99) .. controls (231.67,99) and (216,90.05) .. (216,79) -- cycle ;
%Straight Lines [id:da7175689266618046] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (194,52) -- (225.5,65.92) ;


%Shape: Ellipse [id:dp16958195185242708] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (73,148) .. controls (73,136.95) and (88.67,128) .. (108,128) .. controls (127.33,128) and (143,136.95) .. (143,148) .. controls (143,159.05) and (127.33,168) .. (108,168) .. controls (88.67,168) and (73,159.05) .. (73,148) -- cycle ;
%Straight Lines [id:da825831004548085] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (150,112) -- (108,128) ;


%Straight Lines [id:da48564381269859935] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (218,174) -- (193.5,132.92) ;

% Text Node
\draw (159,52) node   [align=left] {$\displaystyle \textcolor[rgb]{0.11,0.18,0.88}{w_{1}} \dots$};
% Text Node
\draw (220,193) node   [align=left] {$\displaystyle \dots \textcolor[rgb]{0.11,0.18,0.88}{ w_\ell}$};
\end{tikzpicture}
\caption{Acyclic query with two projection variables $w_1$ and $w_\ell$.} \label{fig:acyclic}
\end{figure}

\smallskip
\introparagraph{Data Structure} During the preprocessing phase, we first apply the standard semijoin reduction to remove all the dangling tuples. Then, we pick a relation (arbitrarily) that contains a projection variable and designate it as the root of the decomposition. We can now remove all bags that do not lie on the path between bags containing $w_1$ and $w_\ell$.~\autoref{fig:acyclic} shows the bags removed marked in red. Ror each valuation $v(w_1)$, the data structure $\mds$ stores two things: $(i)$ size of $\tOUT_{\pi}(v(w_1))$; $(ii)$ A list of $|D|/\delta$ answers from $\tOUT_{\pi}(v(w_1))$.

\begin{lemma} \label{lem:space}
	Data structure $\mds$ can be constructed in worst-case time $T = O(|D|^2)$ and uses space at most $S = O(|D|^2/ \delta)$.
\end{lemma}
\begin{proof}
	The semijoin reduction takes time $O(|D|)$. Then, for each valuation $v(w_1)$, we can find $\tOUT_{\pi}(v(w_1))$ by performing $\mbfs$. This takes time $\sum_{v(w_1)} O(|D|) = O(|D|^2)$. The space requirement $S = \sum_{v(w_1)} O(|D|/\delta) = O(|D|^2/\delta)$.
\end{proof}

\smallskip
\introparagraph{Enumeration Phase} During the enumeration phase, for each valuation $v(w_1)$, we check if $|\tOUT_{\pi}(v(w_1))| \leq \mds(v(w_1))$, then we can enumerate the output for $v(w_1)$ with constant delay. Otherwise, we invoke~\autoref{lem:helper:two} with $\mA$ as $\mbfs(v(w_1))$ and $J$ as the stored output for $v(w_1)$. Note that $T = O(|D|)$ and $J = O(|D|/\delta)$ which gives the overall delay as $O(\delta)$.

\subsection{Main Result} \label{subsec:second:space}

In this section, we will improve upon the result of~\autoref{thm:space:one} using a more clever strategy. 

\begin{figure} [hp]
	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
	
	\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,222.921875); %set diagram left start at 0, and has height of 222.921875
	
	%Shape: Ellipse [id:dp3099374396386705] 
	\draw  [color={rgb, 255:red, 11; green, 48; blue, 238 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (28.5,109) .. controls (28.5,97.95) and (47.64,89) .. (71.25,89) .. controls (94.86,89) and (114,97.95) .. (114,109) .. controls (114,120.05) and (94.86,129) .. (71.25,129) .. controls (47.64,129) and (28.5,120.05) .. (28.5,109) -- cycle ;
	%Shape: Ellipse [id:dp7979646113275076] 
	\draw   (61.75,109) .. controls (61.75,97.95) and (80.95,89) .. (104.63,89) .. controls (128.3,89) and (147.5,97.95) .. (147.5,109) .. controls (147.5,120.05) and (128.3,129) .. (104.63,129) .. controls (80.95,129) and (61.75,120.05) .. (61.75,109) -- cycle ;
	%Shape: Ellipse [id:dp7115553367978524] 
	\draw   (84,110) .. controls (84,98.95) and (108.06,90) .. (137.75,90) .. controls (167.44,90) and (191.5,98.95) .. (191.5,110) .. controls (191.5,121.05) and (167.44,130) .. (137.75,130) .. controls (108.06,130) and (84,121.05) .. (84,110) -- cycle ;
	
	% Text Node
	\draw (76,109) node   [align=left] {$\displaystyle \textcolor[rgb]{0.11,0.18,0.88}{w}\textcolor[rgb]{0.11,0.18,0.88}{_{1}}\textcolor[rgb]{0,0,0}{\quad w_{2} \quad w_{3}}$};
	% Text Node
	\draw (206,109) node   [align=left] {$\displaystyle \textcolor[rgb]{0.11,0.18,0.88}{\dots}$};
	% Text Node
	\draw (128,109) node   [align=left] {$\displaystyle w_{4}$};
	% Text Node
	\draw (166,109) node   [align=left] {$\displaystyle w_{5}$};
	% Text Node
	\draw (65,143) node   [align=left] {$\displaystyle R_{1}$};
	% Text Node
	\draw (104,75) node   [align=left] {$\displaystyle R_{2}$};
	% Text Node
	\draw (144,142) node   [align=left] {$\displaystyle R_{3}$};
	
	
	\end{tikzpicture}
	\caption{Acyclic query with $w_1$ as projection variable and $R_1$ as root bag.} \label{fig:improved}
\end{figure}

Without loss of generality, we assume that variables of no relation is contained in another. If this is the case, such relations can be safely deleted after performing semijoin step. Let $\phi_i$ denote the common variables between bags $B_i$ and $B_{i+1}$. For instance, for the query in~\autoref{fig:improved}, $\phi_1 = \{w_2, w_3\}, \phi_2 = \{w_3, w_4\}$ and so on. Let $\phi_0 = \{w_1\}$. We will introduce a degree threshold $\Delta_i$ for each $\phi_i, i \in [k-2]$. We will define a valuation $\bt$ over variables $\phi_i$ to be heavy if $|\sigma_{\phi_i = \bt} B_i| \geq \Delta_i$ and light otherwise. We will store the materialized output for each heavy valuation $\phi_i$ in a recursive manner. 

Suppose that all valuations in all relations are light according to their degree thresholds. Then, for each $v(w_1)$, we can expand $\mL = \pi_{B_1 \cup \dots B_{k-1}} (B_1 {\Join} B_2 {\Join} \dots {\Join} B_k)$  in time $O(\Pi_i \Delta_i)$. Each $t \in \mL$ gives a valuation for $v(w_\ell)$ that can be deduplicated across all $t$ (assuming all relations are indexed and sorted).

Next, we consider each heavy $\phi_i$ valuation reachable from $\phi_0$. Suppose that some $v(w_1)$ is heavy. Then, we will use the data structure from~\autoref{thm:space:one} with $\delta = O(\Pi_{i=1}^{i=k-2}\Delta_i)$. If $v(w_1)$ is light, then there are at most $\Delta_0$ valuations for $\phi_1$ that connect to $v(w_1)$. In order to get the delay guarantee, we need to ensure that for each $\Delta_0$ valuations of $\phi_1$, we can find the connecting projection variable $w_\ell$. This is equivalent to the subquery with bag $B_0$ removed, $w_1 = \phi_1$ and $\delta = O(\Pi_{i=1}^{i=k-2}\Delta_i)$. We can now recursively construct this data structure. The total space requirement of the data structure is
%
\[
S = \frac{|D|}{\Delta_0} \cdot \frac{|D|}{\Delta_0 \dots \Delta_{k-2}} + \frac{|D|}{\Delta_1} \cdot \frac{|D|}{\Delta_1 \dots \Delta_{k-2}} + \dots + \frac{|D|}{\Delta_{k-2}} \cdot \frac{|D|}{\Delta_{k-2}} 
\]
%
and the delay guarantee is $\delta = \Delta_0 \cdot \Delta_1 \cdot \dots \Delta_{k-2}$. The space is minimized when all the terms are equal to each other. This gives $\Delta_{i} = \Delta^2_{i-1}$ for $i \in [1,k-2]$. Thus, space $S = O(|D|/\Delta_0^{2^{k-1}})$ and delay $\delta = O(\Delta_0^{2^{k-1}-1})$.

This gives us the following result.

\begin{theorem} \label{thm:space:two}
	Consider an arbitrary acyclic query $Q$ with at most two projection variables and a database $D$. Then, there exists a data structure that requires space $S = O(|D|^2/\delta^{1 + 1/(2^{k-1}-1)})$ which can be used to enumerate the results of $Q(D)$ with delay $\delta$.
\end{theorem}

\autoref{thm:space:two} is an improvement over~\autoref{thm:space:one} in terms of space usage of the compressed data structure for all $k \geq 2$.




==> spaceresult2.tex <==

\subsection{Hierarchical Queries} \label{subsec:third:space}

\eat{

\begin{theorem} \label{thm:space:star}
	Consider query $\starq$ with factorization width $\mw$ and a database $D$. Then, there exists a data structure that uses space $S = O((|D|/\delta)^\mw)$ and achieves delay $O(\delta)$ during the enumeration phase.
\end{theorem}

\autoref{thm:space:star} is an improvement over~\autoref{thm:basic:three} in terms of space usage. Fixing the value of $\delta = |D|^{1 - \epsilon}$, we can get that $(|D|/\delta)^\mw = |D|^{\epsilon\mw} = |D|^{\epsilon + (w-1)\epsilon} \leq |D|^{1+(w-1)\epsilon}$ since $\epsilon \in [0,1]$. The high level idea of the algorithm is to use~\autoref{lem:merge} for all free variables with degree at most $\delta$ and materialize the output for all heavy valuations.

\smallskip
\introparagraph{Data Structure} As before, we assume that linear time semijoin reduction has already been performed. The preprocessing step will materialize the result of the subquery $Q_k$ where all free variables are heavy.

\begin{lemma}
	Subquery $Q_k$ can be computed in time $O(|D| \cdot (|D|/\delta)^{\mw-1})$ and requires space $S = O((|D|/\delta)^\mw)$ in the worst-case.
\end{lemma}

Note that join $Q_k$ can be stored lexicographically when computing the join (i.e no additional sorting step needed).

\smallskip
\introparagraph{Enumeration} During the enumeration phase, we have subqueries $Q_1, \dots, Q_{k-1}$ and materialized $Q_k$. Each subquery can emit the smallest output result in lexicographic order which can then be compared with the smallest materialized output. The overall smallest output tuple is then returned to the user. Clearly, this achieves delay $O(\delta)$.

\autoref{thm:space:two} and~\autoref{thm:space:star} are both applicable to the two-path query $Q*_2(x,z) = R(x,y),S(y,z)$ which gives two distinct algorithms that lead to the same space-delay tradeoffs. It would be very interesting to compare their performance in practice to see which algorithm performs better based on the dataset used.}

In this section, we will present our main result for hierarchical query $Q$. 

\begin{theorem} \label{thm:space:hierarchical}
	Consider a hierarchical query $Q$ with factorization width $\mw$ and a database $D$. Then, there exists a data structure that uses space $S = O((|D|/\Delta)^\mw)$ such that the delay is $\delta = O(\log|D| \cdot |D|^\mqw/S)$ during the enumeration phase. 
\end{theorem}

In the above theorem, $\Delta$ is the degree threshold for classifying a variable as heavy or light and $\mqw$ is a new notion of query width that depends on the query and $\Delta$. \autoref{thm:space:hierarchical} is an improvement over~\autoref{thm:basic:three} in terms of space usage when $N^\mqw/S = O(\Delta)$. Fixing the value of $\Delta = |D|^{1 - \epsilon}$, we can get that $(|D|/\Delta)^\mw = |D|^{\epsilon\mw} = |D|^{\epsilon + (w-1)\epsilon} \leq |D|^{1+(w-1)\epsilon}$ since $\epsilon \in [0,1]$. As we will see later, this is indeed the case for many queries of practical interest. We will now present some intuition about how the algorithm works. At a high level, the algorithm will follow a similar query partitioning by creating a subquery for any possible instantiation of $Q$ where some free variable is one of $\{h,l\}$ where the degree threshold is $in$. Consider the subquery where all free variables are heavy. In this case, we can simply store the answers directly. This is because there are $O(|D|/\Delta)$ heavy valuations for each free variable and there are at most $\mw$ relations which can contain these variables. Let us now look at the other extreme case, where all free variables are light. In this case, we can partition each relation into blocks of size $O(\Delta)$ taking care that no valuation is split between two blocks. This can always be achieved by increasing the block size by a constant factor. Each relation now has $O(|D|/\Delta)$ blocks in total. During the preprocessing phase, we will store all block combinations(as a list $\mL$) of the form $\langle b_1 \times b_2 \times \dots \times b_\mw \rangle$ that lead to an output tuple. Here, each $b_i$ refers to the index of a block in relation $R_i$. Now we can use~\autoref{prop:basic:two} which guarantees linear delay in the size of the input relations which is $O(\Delta)$ in this case. The correctness follows from the observation that no two block tuples from $\mL$ can lead to a duplicate output. For remaining subqueries, we need to perform some partial materializations so that we can use~\autoref{prop:basic:two}.

We now introduce some notation. Let $\omega$ denote a tree where the vertices are variables of $Q$ and variables of each atom in $Q$ lie along the same root-to-leaf path. Each atom is a child of its lowest variable and the lowest variable is a free variable. The subtree of $\omega$ rooted at a variable $X$ is denoted by $\omega_X$. Given a tree $\omega$ (and similarly for $\omega(X)$) for a query $Q$, we denote by: $\mvars{(\omega)}$ all variables; $\mfree(\omega)$ the free variables; $\matoms(\omega)$ the set of atoms at the leaves. Let $\manc(X)$ the set of variables on the path from a variable $X$ to the root excluding $X$ and $\mparent.X$ denote the parent of $X$ (defined as $\emptyset$ for root). The query at $X$ is denoted by $Q(\mF_X)$: its body is the conjunction of $\matoms(\omega_X)$ and$\mF_X = \mfree(\omega_X) \cup \manc(X) \cup X$. For the remainder of the section, without loss of generality, we assume that linear time semijoin has already been performed, all relations contain at least one free variable and all non-free variables that are present in exactly one relation are removed. We can also remove all relations that are strictly contained in another relation without affecting the correctness of the algorithm. For a given tree $\omega$, each atom is sorted  according to leaf-to-root variable order. Given an annotation $\mann$ for each free variable $Q_\mann$ denotes the subquery where each relation contains tuples that agree with the annotation. Next, we define the query width $\mqw$ of a  query $Q$ for a given $\mann$.

\begin{definition}
	The query width $\mqw$ of an acyclic CQ $Q$, $\omega$, a given $\mann$ and some degree threshold $\Delta$ is
		\begin{align*}
				\mqw(Q_\mann) &= \max_{v \in \omega \setminus \omega.\mroot : \text{all }\mfree(\omega_v) \text{ are heavy}} \log_D |Q_\mann(\mF_v)| \\				
				\mqw(Q) &= \max_{\mann \in \{h,l\}^{|\mfree(Q)|}} \mqw(Q_\mann)
		\end{align*}
\end{definition}

Intuitively, $|D|^\mqw$ tells us the best possible upper bound on time required to compute the join of the largest subquery where all variables are heavy.

\begin{figure}
		\centering
		\begin{tikzpicture}[xscale=1, yscale=1]
		\node at (0.0, 0.0) (A) {{\color{black} $A$}};
		\node at (-1.2, -0.8) (B) {{\color{black} $B$}} edge[-] (A);
		\node at (1.2, -0.8) (C) {{\color{black} $C$}} edge[-] (A);
		\node at (-2.0, -1.6) (D) {{\color{black} $\underline{D}$}} edge[-] (B);
		\node at (-0.7, -1.6) (E) {{\color{black} $\underline{E}$}} edge[-] (B);
		\node at (0.7, -1.6) (F) {{\color{black} $\underline{F}$}} edge[-] (C);
		\node at (2.0, -1.6) (G) {{\color{black} $\underline{G}$}} edge[-] (C);
		\node at (-2.0, -2.4) (R) {{\color{black} $R(AB\underline{D})$}} edge[-] (D);
		\node at (-0.7, -2.4) (S) {{\color{black} $S(AB\underline{E})$}} edge[-] (E);
		\node at (0.7,  -2.4)(T) {{\color{black} $T(AC\underline{F})$}} edge[-] (F);
		\node at (2.0,  -2.4)(U) {{\color{black} $U(AC\underline{G})$}} edge[-] (G);
		\end{tikzpicture}
		\caption{Tree $\omega$ for query $Q(D,E,F,G) = R(A, B, D), S(A, B, E), T (A, C, F),
			U(A, C, G)$} \label{fig:hierarchical:one}
\end{figure}

\begin{example} \label{ex:basic}
	Consider the query $Q(D,E,F,G) = R(A, B, D), S(A, B, E),$ $T (A, C, F),
	U(A, C, G)$ with tree $\omega$ as shown in~\autoref{fig:hierarchical:one}. This query has factorization width $\mw = 4$. Suppose we annotate $\{D,E,F,G\}$ as $\{h,h,l,l\}$ and fix $\Delta = \sqrt{|D|}$. Then all free variables below vertex $B$ are heavy. The join size for the query $Q(B,D,E,A) = R(A,B,D), S(A,B,E)$ is bounded by $|D|^{3/2}$ which gives the width as $3/2$. This is also the largest exponent for all annotations. Thus, $\mqw = 3/2$.
\end{example}

\smallskip
\introparagraph{Preprocessing Phase} This phase comprises of two operations; $(i)$ we annotate each vertex of the tree $\omega$ as $\{\mfm, \mfp\}$: $\mfm$ stands for fully materialized which means that $Q_X(\mF_X)$ needs to be computed during the enumeration phase and $\mfp$ denotes that partitioning of relations is sufficient to perform enumeration of the result during the enumeration phase.~\autoref{algo:hierarchical:preprocessing} describes the preprocessing performed for a specific heavy-light  $\mann \in \{h,l\}^{|\mfree(Q)|}$ of each free variable.

\begin{algorithm}[!htp]
	\SetCommentSty{textsf}
	\DontPrintSemicolon 
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\SetKwFunction{root}{\textsf{root}}
		\SetKwData{lastanswer}{\textsf{lastanswer}}
	\SetKwData{stoppingblock}{\textsf{stoppingblock}}
	\Input{heavy-light annotation of free variables, tree $\omega$, database $D$}
	\Output{Materialized data $M$, $\lastanswer, \stoppingblock$}
	\SetKwData{dedup}{\textsf{dedup}}
	\SetKwData{counter}{\textsf{counter}}
	\For{$v \in \omega$ in post-order traversal}{
		$v.\mlabel= 
		\begin{cases}
			\mfp, & \text{if child is annotated } l\\
			\mfp, & \text{if some child is labelled } \mfp \\
			\mfm, & \text{if all children are annotated } h \\
			\mfm, & \text{if all children are labelled } \mfm \\
		\end{cases}
		$
	}
	
	\tcc{If all free variables are annotated $h$, store $Q(D)$ and return}
	\If{$\omega.\root = \mfm$}{
		$M \leftarrow Q_\mann(D)$ \;
		\textbf{return}
	}
	$\mfree_{\max} \leftarrow \max \{|\mfree(v)| \mid v.\mlabel = \mfm\}$ \;
	\ForEach{$v \in \omega$ such that $v.\mlabel = \mfm$}{
		\label{join:1} Compute $J = Q_\mann(\mF_v)$ and set $v.\mparent[\mfree(w_v)] \leftarrow \pi_{\mfree(w_v) \cup v \cup \manc(v)} (J)$ \;
		\If{$J$ is empty}{
			\textbf{exit} \tcc*{$Q_\mann(D)$ is empty}
		}
	}
	\ForEach{atom $R$ with at least one free variable}{
		Partition into blocks of size $\Theta(\Delta)$ \;
	}
	\tcc{let $\#l$ denote the number of atoms with free variables}
	\ForEach{$B = \langle b_1 \times b_2 \times \dots b_{\#l} \rangle$ in lexicographic order}{
		\label{join:2} Compute $J = Q_\mann \ltimes (b_1, b_2, \dots b_{\#l})$ \;
		\If{$|J| \geq 1$}{$\mL \leftarrow \mL \cup B$ \tcc*{record all blocks with some output}}
		\If{$|M + J| \leq (|D|/\delta)^{\mfree_{\max}} $}{
			$M \leftarrow M \cup J$ \;
		} \Else {
			\If{$|M| \geq  (|D|/\delta)^{\mfree_{\max}} $}{\textbf{break}}
			\ForEach{$t \in J$}{
				\If{$|M| + 1 \leq (|D|/\Delta)^{\mfree_{\max}} $}{$M \leftarrow M \cup t$ \;
					$ \lastanswer \leftarrow t, \stoppingblock \leftarrow B$} \Else {\textbf{break}}
			}
		}
		
	}
	\BlankLine
	\caption{Preprocessing Phase}
	\label{algo:hierarchical:preprocessing}
\end{algorithm}

\begin{lemma}
	\autoref{algo:hierarchical:preprocessing} takes time $O(|D|^\mw)$ and materialized answers $|M| = O((|D|/\Delta)^\mw), |\mL| = O((|D|/\Delta)^\mw)$
\end{lemma}
\begin{proof}
	If all free variables are annotated heavy, then we store $Q_\mann(D)$ and return. Note that there can be at most $O(|D|/\Delta)$ valuations for each heavy free variable and thus, $|Q_\mann(D)| \leq O((|D|/\Delta)^{|\free(Q)|}) = O((|D|/\Delta)^{|\mw|})$.
	The most expensive part of the algorithm is computing the join on~\autoref{join:1} and~\autoref{join:2}.~\autoref{join:1} can take as much as $O(|D|^{\mw-1})$ time for any child of the root vertex (if it labelled $\mfm$).~\autoref{join:2} computes the full join result for the each block tuple $B$. Since each $t \in Q(D)$ can occur in exactly one block $B$, it follows that $\bigcup_B Q \ltimes (b_1, b_2, \dots, b_{\#l}) = Q(D)$ which is at most $O(|D|^\mw)$ in size. The materialized answers $M$ are at most $O((|D|/\Delta)^\mw)$ since it can be the case that $\mfree_{\max} = \mw$ at the root of $\omega$. The claimed bound on size of list of all blocks with some output $\mL$ follows from the observation that each $b_i$ can take at most $\Theta(|D|/\Delta)$ values since each partition block of a relation is of size $\Theta(\Delta)$
\end{proof}

Note that join on~\autoref{join:1} is not materialized in the preprocessing phase. Indeed, the join result for any vertex labeled $\mfm$ can be as large as $O(|D|^\mw)$, which exceeds our space budget. However, we will show that $M$ can be used to compute these joins again on-the-fly while maintaining delay guarantees. 

\begin{figure}
	\centering
	\begin{tikzpicture}[xscale=1, yscale=1]
	\node at (0.0, 0.0) (A) {{\color{black} $A_{\mfp}$}};
	\node at (-1.2, -0.8) (B) {{\color{black} $B_{\mfm}$}} edge[-] (A);
	\node at (1.2, -0.8) (C) {{\color{black} $C_{\mfp}$}} edge[-] (A);
	\node at (-2.0, -1.6) (D) {{\color{black} $\underline{D}$}} edge[-] (B);
	\node at (-0.7, -1.6) (E) {{\color{black} $\underline{E}$}} edge[-] (B);
	\node at (0.7, -1.6) (F) {{\color{black} $\underline{F}$}} edge[-] (C);
	\node at (2.0, -1.6) (G) {{\color{black} $\underline{G}$}} edge[-] (C);
	\node at (-2.0, -2.4) (R) {{\color{black} $R(AB\underline{D})$}} edge[-] (D);
	\node at (-0.7, -2.4) (S) {{\color{black} $S(AB\underline{E})$}} edge[-] (E);
	\node at (0.7,  -2.4)(T) {{\color{black} $T(AC\underline{F})$}} edge[-] (F);
	\node at (2.0,  -2.4)(U) {{\color{black} $U(AC\underline{G})$}} edge[-] (G);
	
	\end{tikzpicture}
	\caption{Labeled tree $\omega$ for query $Q(D,E,F,G) = R(A, B, D), S(A, B, E), T (A, C, F),
		U(A, C, G)$ and $\mann = \{h,h,l,l\}$ for $\langle D,E,F,G \rangle$} \label{fig:hierarchical:two}
\end{figure}

\begin{example} \label{ex:two}
	Continuing with the query from~\autoref{ex:basic},~\autoref{fig:hierarchical:two} shows the labeling of all vertices (except the leaf). $\mfree_{\max} = 2$ since $B$ is the only $\mfm$ labeled vertex. The subtree $Q(A,B,D,E)$ can be computed in time $|D|^{3/2}$ (recall that $D$ and $E$ are heavy) and then $B$ is projected out. Next, we partition the relations $T$ and $U$. Suppose that $\Delta = 2$ and the base relations are as shown below.
	
	\begin{minipage}[t]{0.4\linewidth}
		\centering
		\begin{tabular}[t]{ !{\vrule width1pt} c| c|c|c  !{\vrule width1pt} } 
			\Xhline{1pt}
			$\mathbf{F}$ & $\mathbf{C}$ & $\mathbf{A}$ \\ 
			\Xhline{1pt}
			$f_1$ & 1 & 1 \\ 
			$f_2$ & 1 & 1 \\
			$f_3$ & 2 & 2 \\
			$f_3$ & 3 & 3 \\
			$f_3$ & 4 & 4 \\
			\Xhline{1pt}
		\end{tabular}		
		
		\vspace{1em}
		$T$
	\end{minipage}
	\begin{minipage}[t]{0.4\linewidth}
		\centering
		\begin{tabular}[t]{ !{\vrule width1pt} c| c|c|c !{\vrule width1pt} } 
			\Xhline{1pt}
			$\mathbf{G}$ & $\mathbf{C}$ & $\mathbf{A}$ \\ 
			\Xhline{1pt}
			$g_1$ & 1 & 1 \\ 
			$g_2$ & 1 & 1 \\
			$g_3$ & 2 & 2 \\
			$g_3$ & 3 & 3 \\
			$g_3$ & 4 & 4 \\
			\Xhline{1pt}
		\end{tabular}		

		\vspace{1em}	
		$U$
	\end{minipage}

	Since $\Delta = 2$, only $f_1$ and $f_2$($g_1$ and $g_2$) are light valuations for $T$($U$). There is exactly one block for both relations and the tuples $(f_1,1,1), (f_2,2,2)$ are the members of the block. Similarly for relation $U$, $(g_1,1,1), (g_2,1,1)$ are present in the only block. Suppose that $Q(A,D,E) =\{ (1, d_1, e_1), (1, d_2, e_2), (1, d_3, e_3), (1, d_4, e_4)\}$. The space available is $S = (|D|/\Delta)^2 \approx 4$. Thus, we can store $4$ answer tuples. We start with $f_1$ and see that $g_1, (d_1, e_1), g_1, (d_2, e_2), g_1, (d_3, e_3), g_1, (d_4, e_4)$ are all the answers. Thus, $\mathsf{lastanswer} = (f_1, g_1, (d_4, e_4))$. Since there is only one block pair, $\mL = \mathsf{stoppingblock} = \langle 1 \times 1 \rangle$.
\end{example}


\smallskip
\introparagraph{Enumeration Phase}~\autoref{algo:merging} describes the algorithm for enumeration phase. The first step is to check whether all answers of $Q_\mann(D)$ have been materialized. If they are, we can enumerate them with constant delay and exit the procedure. Otherwise, we use~\autoref{lem:helper:two} to generate $Q_\mann(\mF_v)$ for all vertices of $\omega$ with label $\mfm$. We first show that this can be done while maintaining delay guarantee of $O(\delta)$.

\begin{lemma}
	$Q_\mann(\mF_v)$ for all vertices of $\omega$ with label $\mfm$ can be computed on-the-fly while maintaining delay guarantee of $O(\Delta)$.
\end{lemma}
\begin{proof}
	The first observation is that each $Q_\mann(\mF_v)$ takes time at most $O(|D|^\mqw)$ by definition. In addition to computing $Q_\mann(\mF_v)$, we also want to index and sort them using $v$ as the hash index key and a sorted list of $\free(Q_v)$ as the value. Since we have $S = O((|D|/\Delta)^\mw)$ output available,~\autoref{lem:helper:two} guarantees a delay $\delta = O(\log|D| \cdot |D|^\mqw)/S$. The extra $\log |D|$ factor is to allow for sorting to happen on-the-fly.
\end{proof}

The second step is to continue enumeration from where we stopped during the preprocessing phase. This can be done by using~\autoref{corollary:basic:two} with input relations as the block of tuples of size $O(\Delta)$. This gives us $O(\Delta)$ delay guarantee to find valuations for each light free variable. However, we also need to find valuations for all heavy variables. Our key observation is that~\autoref{corollary:basic:two} already finds the valuations for all variables on leaf to root path. This means that any heavy variable or any $J' = Q_\mann(\mF_v)$ that is attached to this path,~\autoref{algo:merging} is applicable. This is because there are at most $O(\Delta)$ valuations for all variables on leaf to root path and each $J'$ and base relation is already sorted.

\begin{algorithm}[!htp]
	\SetCommentSty{textsf}
	\DontPrintSemicolon 
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\SetKwFunction{enumerate}{\textsf{enumerate}}
	\SetKwProg{Fn}{Function}{}{}
	\SetKwData{lastanswer}{\textsf{lastanswer}}
	\SetKwData{stoppingblock}{\textsf{stoppingblock}}
	\Input{heavy-light annotation of free variables, tree $\omega$, database $D$, Materialized data $M$, $\mL$, $\lastanswer, \stoppingblock$}
	\Output{$Q_\mann(D)$ with $O(\delta)$ delay guarantee}
	\SetKwData{dedup}{\textsf{dedup}}
	\SetKwData{counter}{\textsf{counter}}
	\If{$\stoppingblock == \emptyset$}{
		\tcc{$Q_\mann(D) \leq O((|D|/\delta)^\mw)$}
		Enumerate $M$ with constant delay \;
		\textbf{exit}
	}
	\label{line:gen}Use~\autoref{lem:helper:two} with $J = M$ to compute $J' = Q_\mann(\mF_v)$ and set $v.\mparent[\mfree(w_v) \cup v \cup \manc(v)] \leftarrow \pi_{\mfree(w_v) \cup v \cup \manc(v)} (J')$  for all vertices with $v.\mlabel = \mfm$ \;
	$\enumerate(\omega, \mL, \lastanswer, \stoppingblock)$ \;
	
	\Fn{\enumerate{$\omega, \mL, \lastanswer, \stoppingblock$}}{
		\ForEach{$B \in \mL$ starting from $\stoppingblock$}{
			\If{$B == \stoppingblock$}{
				Use~\autoref{corollary:basic:two} with $t = \lastanswer$ and each relation containing a light variable $R_i \ltimes b_i$. \;
				For each heavy free variable and materialized $Q_\mann(\mF_v)$, use~\autoref{algo:merging}.
			} \Else {
				Use~\autoref{prop:basic:two} with each relation $R_i \ltimes b_i$. \;
				For each heavy free variable and materialized $Q_\mann(\mF_v)$, use~\autoref{algo:merging}.
			}
		}
	}
	\BlankLine
	\caption{Enumeration Phase}
	\label{algo:hierarchical:enumeration}
\end{algorithm}

\begin{example}
	Continuing~\autoref{ex:two}, in order to compute $Q(A,D,E) = R(A,B,D), S(A,B,E)$ when $D,E$ are heavy, we interleave with $M$. The join can be computed in $|D|^{3/2}$ time and we stored $(|D|/\Delta)^2$ time. Therefore, $\delta = O(\log|D| \cdot \Delta)$. By the time we finish enumerating $M$, $Q(A,D,E)$ is sorted and indexed. We now resume the enumeration for $f_1$ since that is where we stopped. In $O(\Delta)$ time, we find that it connects with $g_1, g_2$. For $g_1$, we have enumerated all the output so we move on to $g_2$ which join through $(1,1)$. Since $Q(A,D,E)$ is indexed and sorted, we scan through the list and resume the enumeration.
\end{example}

So far, we have only argued about the delay guarantees for a particular $\mann$ of a hierarchical query $Q$. Since we are interested in data complexity, there are only a constant number of annotations in total (Assuming query size is a constant). Thus, one can record all  $\mann$ that give some output. Note that there is no overlap between materialized answers of any two different subqueries since the join output is partitioned based on the $\mann$.

Another example of hierarchical queries that often occurs in practice are \emph{tall} queries. Here, each relation contains exactly one projection variable (say $w_i$) and the relations form a hierarchy of the following form: $\mvars(R_1) \setminus w_1 \subseteq \mvars(R_2) \setminus w_2 \dots \mvars(R_k) \setminus w_k$. For example, in \textsf{SSB} dataset, \textsf{Lineitem}, \textsf{Partsupp}  contains join keys \textsf{partkey} and \textsf{suppkey} while relation \textsf{Supplier} joins only with \textsf{suppkey}. This is depicted in~\autoref{ex:tall}. It can be verified that for any \emph{tall} query, it holds that $\delta = O(\log |D| \cdot \Delta)$ in~\autoref{thm:space:hierarchical} and thus better than~\autoref{thm:basic:three} for all values of $\Delta$.

\begin{figure}
	\begin{minipage}{0.4\linewidth}
	\scalebox{0.7}{
	\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,222.921875); %set diagram left start at 0, and has height of 222.921875
	
	%Shape: Ellipse [id:dp9946843075284466] 
	\draw   (81.93,7.63) .. controls (95.13,0.57) and (128.14,36.62) .. (155.64,88.13) .. controls (183.15,139.64) and (194.74,187.12) .. (181.53,194.17) .. controls (168.33,201.22) and (135.32,165.18) .. (107.82,113.66) .. controls (80.31,62.15) and (68.72,14.68) .. (81.93,7.63) -- cycle ;
	%Shape: Ellipse [id:dp16621656156041964] 
	\draw   (92.65,26.03) .. controls (110.28,23.81) and (128.55,53.54) .. (133.46,92.44) .. controls (138.36,131.33) and (128.05,164.67) .. (110.42,166.89) .. controls (92.79,169.12) and (74.52,139.39) .. (69.61,100.49) .. controls (64.71,61.59) and (75.02,28.25) .. (92.65,26.03) -- cycle ;
	%Shape: Ellipse [id:dp8861761206505805] 
	\draw   (30.66,73.37) .. controls (25.6,62.08) and (39.92,44.67) .. (62.65,34.49) .. controls (85.38,24.31) and (107.9,25.21) .. (112.96,36.5) .. controls (118.02,47.79) and (103.69,65.2) .. (80.97,75.38) .. controls (58.24,85.56) and (35.72,84.66) .. (30.66,73.37) -- cycle ;
	
	% Text Node
	\draw (164,162) node   [align=left] {$\displaystyle w_{3}$};
	% Text Node
	\draw (102,46) node   [align=left] {$\displaystyle x$};
	% Text Node
	\draw (125,92) node   [align=left] {$\displaystyle y$};
	% Text Node
	\draw (103,144) node   [align=left] {$\displaystyle w_{2}$};
	% Text Node
	\draw (52,64) node   [align=left] {$\displaystyle w_{1}$};
	% Text Node
	\draw (201,198) node   [align=left] {$\displaystyle R_{3}$};
	% Text Node
	\draw (73,163) node   [align=left] {$\displaystyle R_{2}$};
	% Text Node
	\draw (24,43) node   [align=left] {$\displaystyle R_{1}$};
	\end{tikzpicture}}
	\end{minipage}
	\begin{minipage}{0.4\linewidth}
		\scalebox{0.8}{
		\begin{tikzpicture}[xscale=1, yscale=1]
		\node at (0.0, 0.0) (A) {{\color{black} $x$}};
		\node at (-0.7, -0.8) (B) {{\color{black} $\underline{w_1}$}} edge[-] (A);
		\node at (1.2, -0.8) (C) {{\color{black} $y$}} edge[-] (A);
		\node at (0.7, -1.6) (F) {{\color{black} $\underline{w_2}$}} edge[-] (C);
		\node at (2.0, -1.6) (G) {{\color{black} $\underline{w_3}$}} edge[-] (C);
		\end{tikzpicture}}
	\end{minipage}
	\caption{Example of a tall query (left) and its variable tree $\omega$} \label{ex:tall}
\end{figure}
















